Equivariant Cerf theory and perturbative $SU(n)$ Casson invariants

We develop an equivariant Cerf theory for Morse functions on finite-dimensional manifolds with group actions, and adapt the technique to the infinite-dimensional setting to study the moduli space of perturbed flat $SU(n)$-connections. As a consequence, we prove the existence of perturbative $SU(n)$ Casson invariants on integer homology spheres for all $n\ge 3$, and write down an explicit formula when $n=4$. This generalizes the previous works of Boden and Herald.

==> bifurcation.tex <==
%!TEX root = casson.tex
Although the previous section proves general statements for all compact, simple and simply-connected Lie groups, we focus on the case when $G = \SU(n)$ from now on. In this section, we take on the task of analyzing all possible irreducible bifurcations when one varies the perturbation parameter $h \in \mathcal{H}$ along a generic path. In the first part, we list degenerations of $\SU(n)-$connections and their stabilizers. Moreover, we classify symmetry-breaking bifurcations from a given stratum, based on representation-theoretic considerations. In the second part, we discuss about the orientations of moduli spaces, (equivariant) spectral flows of self-adjoint operators. These discussions combined with the results in finite dimensions lead us to a definition of $\SU(n)-$Casson invariant, modulo the elimination of gauge ambiguity. All the arguments are exercises on linear algebra.
\subsection{$\SU(n)$--flat connections and bifurcations}

Throughout this section, we do not consider the trivial product connection. Using the standard linear action of $\SU(n)$ on $\bC^n$, the principal $\SU(n)-$bundle $P$ defines a rank $n$ vector bundle $E$ on $Y$. An $\SU(n)-$connection $A$ is irreducible if and only if its stabilizer is given by the center of $\SU(n)$, which is isomorphic to $\bZ \slash n$. When the connection $A$ is reducible, we can find unitary $\bC-$vector bundles $E(n_1), \dots, E(n_r)$ of ranks $n_1, \dots, n_r$, and integers $m_1, \dots, m_r \geq 1$, such that we have the isomorphism
\begin{equation}
\label{eqn:split}
E \cong \oplus_{i=1}^{r} E(n_i)^{\oplus m_i}
\end{equation}
and the induced connection on $E$ respects this splitting. We introduce some further notations to study reducible connections. Let $\U(n_i)_{m_i}$ be the diagonal embedding of $\U(n_i)$ into the product group $\U(n_i)^{m_i}$. If $A$ preserves the splitting \eqref{eqn:split}, then the holonomy group of $A$, written as $\hol_{Y}(A)$, is conjugate to a subgroup of
\[ \s (\U(n_1)_{m_1} \times \cdots \times \U(n_r)_{m_r}), \]
and the symbol $\s$ in the front means that we consider unitary matrices of determinant $1$.

The stabilizer of $A$ under the action of the full gauge group $\mathcal{G}$, or equivalently the stabilizer of $[A] \in \tilde{\mathcal{B}}$ under the action of $\SU(n)$, is identified with the centralizer of the holonomy group $\hol_{Y}(A)$ in $\SU(n)$. If we further require that the connection does not preserve any further splitting of \eqref{eqn:split}, using the same reduction as in the previous paragraph, we can see that $\Stab([A])$ is isomorphic to 
\begin{equation}
\label{eqn:stab}
\s (\U(m_1) \times \cdots \times \U(m_r)). 
\end{equation}
This group is realized as a subgroup of $\SU(n)$ as follows. First we consider the group $\U(m_i n_i)$, viewed as the group of $m_i n_i \times m_i n_i$ unitary matrices. We write these matrices in the block form
\[ \begin{pmatrix}
U^{(i)}_{11} & U^{(i)}_{12} & \dots & U^{(i)}_{1m_{i}} \\
U^{(i)}_{21} & U^{(i)}_{22} & \dots & U^{(i)}_{2m_{i}} \\
\vdots & \vdots & \ddots & \vdots \\
U^{(i)}_{m_i 1} & U^{(i)}_{m_i 2} & \dots & U^{(i)}_{m_i m_{i}}
\end{pmatrix}, \]
where the entries are $n_i \times n_i$ matrices. Then $\U(m_i)$ is realized as a subgroup of $\U(m_i n_i)$ by mapping $(u_{pq})_{m_i \times m_i} \in \U(m_i)$ to
\[ \begin{pmatrix}
u_{11} \cdot \id & u_{12} \cdot \id & \dots & u_{1 m_i} \cdot \id \\
u_{21} \cdot \id & u_{2} \cdot \id & \dots & u_{2 m_i} \cdot \id \\
\vdots & \vdots & \ddots & \vdots \\
u_{m_i 1} \cdot \id & u_{m_i 2} \cdot \id& \dots & u_{m_i m_i} \cdot \id
\end{pmatrix} \]
and $\id$ stands for the $n_i \times n_i$ identity matrix. Next, $\U(m_1 n_1) \times \cdots \times \U(m_r n_r)$ is realized as a subgroup of $\U(n)$ by block-diagonal matrices: 
\[ \diag(U^{(1)}, \dots, U^{(r)}), U^{(i)} \in \U(m_i n_i). \]
The composition of these two steps embeds $\U(m_1) \times \cdots \times \U(m_r)$ as a subgroup of $\U(n)$. Lastly, if we take the intersection between this subgroup and the subgroup $\SU(n) \subset \U(n)$, we get the group \eqref{eqn:stab}. Note that the symbol $\s$ in the front is not being determinant-$1$ and we apologize for possible confusions.

\begin{remark}
When $Y$ is an integer homology sphere, every flat complex line bundle over $Y$ is necessarily trivial. If we restrict ourselves to small perturbations, certain strata will not show up in the perturbed-flat moduli space of framed connections.
\end{remark}

Let $I_n$ be the index set above. The stratification defines a partial order on the set $I_n$: for $\kappa_1, \kappa_2 \in I_n$, let $\kappa_1 \prec \kappa_2$ if $\tilde{\mathcal{B}}_{\kappa_1} \subset \overline{\tilde{\mathcal{B}}_{\kappa_2}}$. Let the isomorphism classes of the corresponding stabilizers be $[G_{\kappa_1}]$ and $[G_{\kappa_2}]$. For the analysis of bifurcations, we need a refinement of this partial order. 

\begin{Definition}
\label{defn:next}
For $\kappa_1, \kappa_2 \in I_n$ such that $\kappa_1 \prec \kappa_2$, we say that $\kappa_1$ is \emph{next to} $\kappa_2$, written as $\kappa_1 \rightarrow \kappa_2$, if the pair $([G_{\kappa_1}], [G_{\kappa_2}])$ appears in a generic one-parameter family of perturbation data. MAKE NEW DEFINITION IN SECTION 2. 
\end{Definition}

Let us pause here to explain our purpose of subsection further. Given two perturbation data $h_0, h_1 \in \mathcal{H}$ lying in different "chambers" of the space $\mathcal{H}$, we can assume that they are connected via a path $h_t$ just passing through one wall $\mathcal{H}([H], (1), V)$ transversely without any loss generality by Corollary \ref{cor:4.14}. When $W$ is a non-trivial irreducible representation of the group $H$, perturbed flat connections with smaller stabilizers might be created or killed during this deformation process. We would like to understand what the representations $W$ would be, provided we know about the group $H$. Moreover, we would like to determine the stabilizers of those "less reducible" connections/critical points which are created or killed during this specific bifurcation process.

Suppose that $[A] \in \tilde{\mathcal{B}}$ is a point with datum $((n_1, m_1), \dots, (n_r, m_r))$. Without loss of generality, let the holonomy group of $A$ be $\s (\U(n_1)_{m_1} \times \cdots \times \U(n_r)_{m_r})$. Using the Killing form, the orthogonal complement of the Lie algebra of $\hol_{Y}(A)$, written as $\mathfrak{g}_A^{\perp}$, is spanned by the following traceless matrices 
\begin{equation}
\begin{pmatrix}
W_{11} & W_{12} & \dots & W_{1r}  \\
W_{21} & W_{22} & \dots & W_{2r}  \\
\vdots & \vdots & \ddots & \vdots \\
W_{r1} & W_{r2} & \dots & W_{rr}
\end{pmatrix},
\end{equation}
such that: for $1 \leq p, q \leq r$,
\begin{itemize}
\item if $p \neq q$, $W_{pq}$ is a $\bC-$valued $m_p n_p \times m_q n_q$ matrix, and $W_{pq} = W_{qp}^*$;
\item if $p = q$ and we write $W_{pp}$ as
\[
\begin{pmatrix}
W^{(p)}_{11} & W^{(p)}_{12} & \dots & W^{(p)}_{1m_{p}} \\
W^{(p)}_{21} & W^{(p)}_{22} & \dots & W^{(p)}_{2m_{p}} \\
\vdots & \vdots & \ddots & \vdots \\
W^{(p)}_{m_p 1} & W^{(p)}_{m_p 2} & \dots & W^{(p)}_{m_p m_{p}}
\end{pmatrix}, \]
then $W^{(p)}_{11}, \dots, W^{(p)}_{m_p m_{p}} \in \mathfrak{su}(n_p)$ and $W^{(p)}_{11} + \dots + W^{(p)}_{m_p m_{p}} = 0$; moreover $W^{(p)}_{i_1, i_2}$ is an $n_p \times n_p$ $\bC-$valued matrix and $W^{(p)}_{i_1, i_2} = (W^{(p)}_{i_2, i_1})^{*}$ for $i_1 \neq i_2$.
\end{itemize}
The group from equation $\eqref{eqn:stab}$ without determinant constraints $U(m_1) \times \cdots \times \U(m_r)$ acts on $\mathfrak{g}_A^{\perp}$ by conjugation. This is just the restriction of the adjoint representation. It is easy to see that each diagonal block $W_{pp}$ and each pair of off-diagonal blocks $(W_{pq,} W_{qp})$ are invariant subspaces under the action of $U(m_1) \times \cdots \times \U(m_r)$. To be more specific, we have the following observations:
\begin{itemize}
\item The action of $U(m_1) \times \cdots \times \U(m_r)$ on the diagonal blocks $W_{pp}, 1 \leq p \leq r$ factors through the projection to the $p-$th coordinate $U(m_p)$. Such a representation, after projecting as a representation of $U(m_p)$, is isomorphic to $n_{p}^2$ copies of the adjoint representation of $U(m_p)$ on $\mathfrak{su}(m_p)$.
\item The action of $U(m_1) \times \cdots \times \U(m_r)$ on the off-diagonal blocks $(W_{pq,} W_{qp})$ factors through the projection to $U(m_p) \times \U(m_q)$. Such a representation, as a representation of the group $U(m_p) \times \U(m_q)$, is isomorphic to $n_p n_q$ copies of the standard representation on $\mat_{m_p \times m_q}(\bC)$, mapping $M$ to $U_1 M U_2^*$ for $U_1 \in U(m_p)$ and $U_2 \in U(m_q)$.
\end{itemize}

After restricting these actions back to the group $\s (\U(m_1) \times \cdots \times \U(m_r))$, the above still gives an isotypic decomposition of $\mathfrak{g}_{A}^{\perp}$. Combining with the discussion in Section 4, we arrive at:

\begin{Lemma}
Let $([A], h) \in \mathcal{H}([H], (1), V)$ as a generic point for $H \cong \s (\U(m_1) \times \cdots \times \U(m_r))$. If $V$ is not the trivial representation, then $V \cong\mathfrak{su}(m_p)$ or $V \cong \mat_{m_p \times m_q}(\bC)$, via the action described above.

ADD DISCUSSIONS ON GENERIC POINTS ON THE WALL.
\end{Lemma}
\begin{proof}
The cohomology group $H^{1}_{A}(Y;\mathfrak{su}(n))$, as a $\Stab([A])-$vector space, is a sub-representation of the $\Stab([A])-$vector space $\Omega_{Y}^{1}(\mathfrak{su}(n)) \cong \Omega_{Y}^{1} \otimes \mathfrak{su}(n)$. The lemma follows from the non-triviality assumption on $W$ and previous discussions.
\end{proof}

With these preparations, we establish a necessary condition for all $\kappa_2 \in I_n$ such that $\kappa_1$ is next to $\kappa_2$ for a given $\kappa_1 \in I_n$, c.f. Definition \ref{defn:next}. Again this is elementary linear algebra. Using the Kuranishi reduction, it suffices to determine the isomorphism types of stabilizers of the $U(m_p)-$space $\mathfrak{su}(m_p)$ and the $U(m_p) \times \U(m_q)-$space $\mat_{m_p \times m_q}(\bC)$, using the linear action described above.

In the case of the adjoint action, because every matrix in $\mathfrak{su}(m_p)$ is normal, the stabilizer of each element is determined by the partition type of its eigenvalues. Namely, if $W^{(p)} \in \mathfrak{su}(m_p)$ and the multiplicities of its eigenvalue are given by $(m_{1}^{(p)}, \dots, m_{r}^{(p)})$, then its stabilizer in $\U(m_p)$ is conjugate to $\U(m_{1}^{(p)}) \times \cdots \times \U(m_{r}^{(p)})$.

In the case of the action of the group $U(m_p) \times \U(m_q)$, the discussion is an application of the singular value decomposition(SVD).  Without loss of generality, let us assume that $m_p \leq m_q$. Then the SVD implies that every matrix $W^{(p,q)} \in \mat_{m_p \times m_q}(\bC)$ is equivalent to the matrix
\[
\begin{pmatrix}
\mu_{1} & 0 & \dots & 0 & | & 0 & \dots & 0 \\
0 & \mu_{2} & \dots & 0 & | & 0 & \dots & 0 \\
\dots & \dots & \dots & \dots & | & 0 & \dots & 0 \\
0 & 0 & \dots & \mu_{m_p} & | & 0 & \dots & 0 \\
\end{pmatrix},
\]
such that $\mu_{1} \geq \mu_{2} \geq \cdots \geq \mu_{m_p} \geq 0$ are the singular values of the matrix $W^{(p,q)}$. There are two cases to consider.
\begin{itemize}
\item If $\mu_{m_p} > 0$, let the multiplicities of the singular values be $(m_{1}^{(p,q)}, \dots, m_{j}^{(p,q)})$. Then the stabilizer of $W^{(p,q)}$ is isomorphic to $\U(m_{1}^{(p,q)}) \times \cdots \times \U(m_{j}^{(p,q)}) \times \U(m_q - m_p)$. This is embedded as a subgroup of $U(m_p) \times \U(m_q)$ by mapping $(U_1, \dots, U_j, U_{j+1})$ to the pair of matrices 
\[ \diag(U_1, \dots, U_j), \diag(U_1, \dots, U_j, U_{j+1}). \]

\item If $\mu_{m_p} = 0$, let the multiplicities of the non-zero singular values be $(m_{1}^{(p,q)}, \dots, m_{j-1}^{(p,q)})$ and the multiplicity of $0$ be $m_{j}^{(p,q)}$. Then the stabilizer of $W^{(p,q)}$ is isomorphic to $\U(m_{1}^{(p,q)}) \times \cdots \times \U(m_{j-1}^{(p,q)}) \times \U(m_{j}^{(p,q)})  \times \U(m_q - m_p + m_{j}^{(p,q)})$. This is embedded as a subgroup of $U(m_p) \times \U(m_q)$ by mapping $(U_1, \dots, U_j, U_{j+1})$ to the pair of matrices 
\[ \diag(U_1, \dots, U_j), \diag(U_1, \dots, U_{j-1}, U_{j+1}). \]
\end{itemize}

Taking the centralizer of the stabilizer, we get back the holonomy group of the connection. Therefore, the arguments could be summarized in the following proposition.

\begin{Proposition}
Let $[A] \in \tilde{\mathcal{B}}$ belong to the stratum indexed by $((n_1, m_1), \dots, (n_r, m_r))$. The indices in $I_n$ which are next to $((n_1, m_1), \dots, (n_r, m_r))$ must satisfy (reorder so that the nondecreasing condition is satisfied)
\begin{itemize}
\item replacing the pair $(n_p, m_p)$ for some $1 \leq p \leq r$ by $((n_p, m_{1}^{(p)}), \dots, (n_p, m_{j}^{(p)}))$ with $m_p = m_{1}^{(p)} + \cdots m_{j}^{(p)}$,
\item or replacing the two-tuple of pairs $((n_p, m_p), (n_q, m_q))$ for some $1 \leq p \neq q \leq r$ and $m_p \leq m_q$ by $((n_q, m_q - m_p), (n_p + n_q, m_{1}^{(p,q)}), \dots, (n_p + n_q, m_{j}^{(p,q)}))$, or $((n_p, m_{j}^{(p,q)}),(n_q, m_q - m_p),(n_p + n_q, m_{1}^{(p,q)}), \dots, (n_p + n_q, m_{j-1}^{(p,q)}))$ also with $m_p = m_{1}^{(p,q)} + \cdots m_{j}^{(p,q)}$.
\end{itemize}
\end{Proposition}

As an example, let us consider the case when $Y$ is an integer homology sphere and $n = 4$, which appeared in \cite{herald2006transversality}. Note that in this case, there are no non-trivial flat line bundles. The same result holds for critical points of the perturbed functional $\CS + h$ if the perturbation $h$ is sufficiently small. Then the set of partitions of $4$ we need to consider is
\[ \{((4,1)), ((1,1), (3,1)), ((2,1), (2,1)), ((2,2)), ((1, 2), (2,1)) \}. \]
The complete relations of one element being next to another are given by
\[ ((1,1), (3,1)) \rightarrow ((4,1)), ((2,1), (2,1)) \rightarrow ((4,1)), \]
\[ ((2,2)) \rightarrow ((2,1), (2,1)), ((1, 2), (2,1)) \rightarrow ((1,1), (3,1)). \]
\subsection{Spectral flows and equivariant Cerf diagrams}
